High-Speed Motion Planning for Aerial Swarms in Unknown and Cluttered Environments

Coordinated flight of multiple drones allows to achieve tasks faster such as search and rescue and infrastructure inspection. Thus, pushing the state-of-the-art of aerial swarms in navigation speed and robustness is of tremendous benefit. In particular, being able to account for unexplored/unknown environments when planning trajectories allows for safer flight. In this work, we propose the first high-speed, decentralized, and synchronous motion planning framework (HDSM) for an aerial swarm that explicitly takes into account the unknown/undiscovered parts of the environment. The proposed approach generates an optimized trajectory for each planning agent that avoids obstacles and other planning agents while moving and exploring the environment. The only global information that each agent has is the target location. The generated trajectory is high-speed, safe from unexplored spaces, and brings the agent closer to its goal. The proposed method outperforms four recent state-of-the-art methods in success rate (100% success in reaching the target location), flight speed (97% faster), and flight time (50% lower). Finally, the method is validated on a set of Crazyflie nano-drones as a proof of concept.

==> tikz_diagrams/docs/0ce53c08-d104-403e-a9e0-deac4932de13 <==
{"id":"r0.1436167426067747","lines":[{"id":"n0.24770977733770372","blocks":[]},{"id":"n0.5385057710292174","blocks":[{"id":"n0.0737683225316601","text":"\\diagram","type":"composite","elements":{"de6174325014134867":{"id":"de6174325014134867","lines":[{"id":"n0.6180262773012111","blocks":[{"id":"n0.8249250269769637","text":"JPS"}]}],"shape":{"data":{"p":{"x":362.99267578125,"y":179}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isTextMode":true},"de47786157725200296":{"id":"de47786157725200296","lines":[{"blocks":[{"id":"n0.7528737694817138","text":"Path shortening"}],"id":"n0.1053396881454911"}],"shape":{"data":{"p":{"x":732,"y":179}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isTextMode":true},"de9124359595355367":{"id":"de9124359595355367","lines":[{"blocks":[{"id":"n0.5478618347418478","text":"DMP"}],"id":"n0.8910779679376135"}],"shape":{"data":{"p":{"x":543.246337890625,"y":179}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isTextMode":true},"de20839015266934946":{"id":"de20839015266934946","lines":[{"blocks":[{"id":"n0.41838872468772137","text":"Occupied"}],"id":"n0.3544756109671454"}],"shape":{"data":{"p":{"x":-161,"y":179}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isTextMode":true},"de6563392853627945":{"id":"de6563392853627945","lines":[{"blocks":[{"id":"n0.08529044190471868","text":"Potential Field"}],"id":"n0.17400840337001866"}],"shape":{"data":{"p":{"x":49,"y":179}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isTextMode":true}},"connections":[],"intersections":{"id":"di6469837643957062","items":[],"style":{}},"shapes":[{"id":"dp9995335108247907","type":"square","data":{"p1":{"x":128,"y":391},"p2":{"x":178,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6588805852312478","type":"square","data":{"p1":{"x":178,"y":391},"p2":{"x":228,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6377929939142277","type":"square","data":{"p1":{"x":228,"y":391},"p2":{"x":278,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5690235729825306","type":"square","data":{"p1":{"x":278,"y":391},"p2":{"x":328,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5648175444951244","type":"square","data":{"p1":{"x":328,"y":391},"p2":{"x":378,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3141830831064576","type":"square","data":{"p1":{"x":378,"y":391},"p2":{"x":428,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp924566917352317","type":"square","data":{"p1":{"x":428,"y":391},"p2":{"x":478,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9812447226369865","type":"square","data":{"p1":{"x":478,"y":391},"p2":{"x":528,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp018587104292868917","type":"square","data":{"p1":{"x":525,"y":391},"p2":{"x":575,"y":441}},"style":{"fillColor":[255,255,255,1]}},{"id":"da22433275914983053","data":[{"x":-147,"y":416},{"x":900,"y":416}],"head":"no","tail":"no","shaft":"|","mVer":1,"style":{"thickness":5,"strokeColor":[139,87,42,1]},"settings":{"separatorDistance":34,"separatorLength":19}},{"id":"dg07033496375516757","entities":[{"id":"dp5997894871093403","type":"rectangle","data":{"p1":{"x":162,"y":-80},"p2":{"x":253,"y":11}}},{"id":"dp3381993608178069","type":"rectangle","data":{"p1":{"x":253,"y":-80},"p2":{"x":344,"y":11}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp7277359316712408","type":"rectangle","data":{"p1":{"x":162,"y":-171},"p2":{"x":253,"y":-80}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp4746369818920202","type":"rectangle","data":{"p1":{"x":253,"y":-171},"p2":{"x":344,"y":-80}}},{"id":"da678786090592701","data":[{"x":207.5,"y":-34.5},{"x":298.5,"y":-125.5}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2},"headScale":1},{"id":"da40089293704229045","data":[{"x":207.5,"y":-34.5},{"x":298.5,"y":-34.5},{"x":298.5,"y":-125.5}],"head":">","tail":"no","shaft":"--","mVer":1,"middle":"no","style":{"strokeColor":[126,211,33,1],"thickness":2},"headScale":1},{"id":"da011745307779843728","data":[{"x":207.5,"y":-34.5},{"x":207.5,"y":-125.5},{"x":298.5,"y":-125.5}],"head":">","tail":"no","shaft":"--","mVer":1,"middle":"no","style":{"strokeColor":[126,211,33,1],"thickness":2},"headScale":1}],"data":{}},{"id":"dp7487585294057495","type":"square","data":{"p1":{"x":-222,"y":241},"p2":{"x":-172,"y":291}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp47772218022841617","type":"square","data":{"p1":{"x":-222,"y":291},"p2":{"x":-172,"y":341}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8067594819677548","type":"square","data":{"p1":{"x":-172,"y":291},"p2":{"x":-122,"y":341}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp3271702411784483","type":"square","data":{"p1":{"x":-172,"y":241},"p2":{"x":-122,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp4242998295667386","type":"square","data":{"p1":{"x":-122,"y":241},"p2":{"x":-72,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp8723085969977997","type":"square","data":{"p1":{"x":-122,"y":291},"p2":{"x":-72,"y":341}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp3822235847042801","type":"square","data":{"p1":{"x":-72,"y":291},"p2":{"x":-22,"y":341}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp7383389489649317","type":"square","data":{"p1":{"x":-72,"y":241},"p2":{"x":-22,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp23073433702602242","type":"square","data":{"p1":{"x":-222,"y":341},"p2":{"x":-172,"y":391}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp9521594596195948","type":"square","data":{"p1":{"x":-222,"y":391},"p2":{"x":-172,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp9715806471217054","type":"square","data":{"p1":{"x":-172,"y":391},"p2":{"x":-122,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp04302787803111863","type":"square","data":{"p1":{"x":-172,"y":341},"p2":{"x":-122,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp8657711958971239","type":"square","data":{"p1":{"x":-122,"y":341},"p2":{"x":-72,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp6419699727421306","type":"square","data":{"p1":{"x":-122,"y":391},"p2":{"x":-72,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7114695086382592","type":"square","data":{"p1":{"x":-72,"y":391},"p2":{"x":-22,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7457673161123579","type":"square","data":{"p1":{"x":-22,"y":241},"p2":{"x":28,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp22835841157564762","type":"square","data":{"p1":{"x":-22,"y":291},"p2":{"x":28,"y":341}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp37495957099999644","type":"square","data":{"p1":{"x":28,"y":291},"p2":{"x":78,"y":341}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp4164228509515133","type":"square","data":{"p1":{"x":28,"y":241},"p2":{"x":78,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp4119681548641958","type":"square","data":{"p1":{"x":78,"y":241},"p2":{"x":128,"y":291}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp3320721792672563","type":"square","data":{"p1":{"x":78,"y":291},"p2":{"x":128,"y":341}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7029758167959068","type":"square","data":{"p1":{"x":128,"y":291},"p2":{"x":178,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9332778491655698","type":"square","data":{"p1":{"x":128,"y":241},"p2":{"x":178,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9234048954551273","type":"square","data":{"p1":{"x":-22,"y":341},"p2":{"x":28,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp9364732416356376","type":"square","data":{"p1":{"x":-22,"y":391},"p2":{"x":28,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp5612922368603566","type":"square","data":{"p1":{"x":28,"y":391},"p2":{"x":78,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7398211794947496","type":"square","data":{"p1":{"x":28,"y":341},"p2":{"x":78,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp024815941488651072","type":"square","data":{"p1":{"x":78,"y":341},"p2":{"x":128,"y":391}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp21736068120312746","type":"square","data":{"p1":{"x":78,"y":391},"p2":{"x":128,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp9728499880462278","type":"square","data":{"p1":{"x":128,"y":341},"p2":{"x":178,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7883682023960088","type":"square","data":{"p1":{"x":-222,"y":441},"p2":{"x":-172,"y":491}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8076530686167611","type":"square","data":{"p1":{"x":-222,"y":491},"p2":{"x":-172,"y":541}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp9472651432439689","type":"square","data":{"p1":{"x":-172,"y":491},"p2":{"x":-122,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp8558205252825084","type":"square","data":{"p1":{"x":-172,"y":441},"p2":{"x":-122,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp52123316192484","type":"square","data":{"p1":{"x":-122,"y":441},"p2":{"x":-72,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp39846244103871675","type":"square","data":{"p1":{"x":-122,"y":491},"p2":{"x":-72,"y":541}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp3115216106266121","type":"square","data":{"p1":{"x":-72,"y":491},"p2":{"x":-22,"y":541}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp43325236781668797","type":"square","data":{"p1":{"x":-72,"y":441},"p2":{"x":-22,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp20263577370793406","type":"square","data":{"p1":{"x":-222,"y":541},"p2":{"x":-172,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8557029395472511","type":"square","data":{"p1":{"x":-222,"y":591},"p2":{"x":-172,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp012579789342798797","type":"square","data":{"p1":{"x":-172,"y":591},"p2":{"x":-122,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7072440894456384","type":"square","data":{"p1":{"x":-172,"y":541},"p2":{"x":-122,"y":591}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp607149979732486","type":"square","data":{"p1":{"x":-122,"y":541},"p2":{"x":-72,"y":591}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp7604625135688841","type":"square","data":{"p1":{"x":-122,"y":591},"p2":{"x":-72,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp06450668408100846","type":"square","data":{"p1":{"x":-72,"y":591},"p2":{"x":-22,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp07753643485044281","type":"square","data":{"p1":{"x":-72,"y":541},"p2":{"x":-22,"y":591}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp5913340543543595","type":"square","data":{"p1":{"x":-22,"y":441},"p2":{"x":28,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp22975429818627657","type":"square","data":{"p1":{"x":-22,"y":491},"p2":{"x":28,"y":541}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp41942558015518494","type":"square","data":{"p1":{"x":28,"y":491},"p2":{"x":78,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp07476571326995907","type":"square","data":{"p1":{"x":28,"y":441},"p2":{"x":78,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp9781898865880563","type":"square","data":{"p1":{"x":78,"y":441},"p2":{"x":128,"y":491}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp21271561050807453","type":"square","data":{"p1":{"x":78,"y":491},"p2":{"x":128,"y":541}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7468537628583956","type":"square","data":{"p1":{"x":128,"y":491},"p2":{"x":178,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp36558566466925746","type":"square","data":{"p1":{"x":128,"y":441},"p2":{"x":178,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6531139343775385","type":"square","data":{"p1":{"x":-22,"y":541},"p2":{"x":28,"y":591}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp08864754165155198","type":"square","data":{"p1":{"x":-22,"y":591},"p2":{"x":28,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp08595891646630305","type":"square","data":{"p1":{"x":28,"y":591},"p2":{"x":78,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp793875073802329","type":"square","data":{"p1":{"x":28,"y":541},"p2":{"x":78,"y":591}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp015199288199182925","type":"square","data":{"p1":{"x":78,"y":541},"p2":{"x":128,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp09290932076692093","type":"square","data":{"p1":{"x":78,"y":591},"p2":{"x":128,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp4861587771885265","type":"square","data":{"p1":{"x":128,"y":591},"p2":{"x":178,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp24903766274810835","type":"square","data":{"p1":{"x":128,"y":541},"p2":{"x":178,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6627135174708092","type":"square","data":{"p1":{"x":178,"y":241},"p2":{"x":228,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp2617834608009828","type":"square","data":{"p1":{"x":178,"y":291},"p2":{"x":228,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5513786559549341","type":"square","data":{"p1":{"x":228,"y":291},"p2":{"x":278,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4447209536925183","type":"square","data":{"p1":{"x":228,"y":241},"p2":{"x":278,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7246445740969232","type":"square","data":{"p1":{"x":278,"y":241},"p2":{"x":328,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp24936389529715153","type":"square","data":{"p1":{"x":278,"y":291},"p2":{"x":328,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9928308094357212","type":"square","data":{"p1":{"x":328,"y":291},"p2":{"x":378,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp22167217417795482","type":"square","data":{"p1":{"x":328,"y":241},"p2":{"x":378,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3860935737662674","type":"square","data":{"p1":{"x":178,"y":341},"p2":{"x":228,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8523196959205939","type":"square","data":{"p1":{"x":228,"y":341},"p2":{"x":278,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9758978489038908","type":"square","data":{"p1":{"x":278,"y":341},"p2":{"x":328,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp12677444577306862","type":"square","data":{"p1":{"x":328,"y":341},"p2":{"x":378,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp32862137479870057","type":"square","data":{"p1":{"x":378,"y":241},"p2":{"x":428,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4106952089198723","type":"square","data":{"p1":{"x":378,"y":291},"p2":{"x":428,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4551264389899783","type":"square","data":{"p1":{"x":428,"y":291},"p2":{"x":478,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp13628092373841194","type":"square","data":{"p1":{"x":428,"y":241},"p2":{"x":478,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp03439395068248108","type":"square","data":{"p1":{"x":478,"y":241},"p2":{"x":528,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp23220206115509212","type":"square","data":{"p1":{"x":478,"y":291},"p2":{"x":528,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5300202016095179","type":"square","data":{"p1":{"x":525,"y":291},"p2":{"x":575,"y":341}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp14742524613944985","type":"square","data":{"p1":{"x":525,"y":241},"p2":{"x":575,"y":291}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7993255177025809","type":"square","data":{"p1":{"x":378,"y":341},"p2":{"x":428,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7452237615807871","type":"square","data":{"p1":{"x":428,"y":341},"p2":{"x":478,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp06825116419048127","type":"square","data":{"p1":{"x":478,"y":341},"p2":{"x":528,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3936059005570891","type":"square","data":{"p1":{"x":525,"y":341},"p2":{"x":575,"y":391}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp36277165863417715","type":"square","data":{"p1":{"x":178,"y":441},"p2":{"x":228,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4238903916444341","type":"square","data":{"p1":{"x":178,"y":491},"p2":{"x":228,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp43465869087842424","type":"square","data":{"p1":{"x":228,"y":491},"p2":{"x":278,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp04582262434058726","type":"square","data":{"p1":{"x":228,"y":441},"p2":{"x":278,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp21056643924633844","type":"square","data":{"p1":{"x":278,"y":441},"p2":{"x":328,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8988667541427171","type":"square","data":{"p1":{"x":278,"y":491},"p2":{"x":328,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3258638980627766","type":"square","data":{"p1":{"x":328,"y":491},"p2":{"x":378,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp518130802468608","type":"square","data":{"p1":{"x":328,"y":441},"p2":{"x":378,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp35680443634927683","type":"square","data":{"p1":{"x":178,"y":541},"p2":{"x":228,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3171092937078408","type":"square","data":{"p1":{"x":178,"y":591},"p2":{"x":228,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp21463873821459822","type":"square","data":{"p1":{"x":228,"y":591},"p2":{"x":278,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6416436152620761","type":"square","data":{"p1":{"x":228,"y":541},"p2":{"x":278,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp004632780152900695","type":"square","data":{"p1":{"x":278,"y":541},"p2":{"x":328,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9439628519076189","type":"square","data":{"p1":{"x":278,"y":591},"p2":{"x":328,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5786420575633089","type":"square","data":{"p1":{"x":328,"y":591},"p2":{"x":378,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp08632331510139846","type":"square","data":{"p1":{"x":328,"y":541},"p2":{"x":378,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7945490225092415","type":"square","data":{"p1":{"x":378,"y":441},"p2":{"x":428,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp2905820119724738","type":"square","data":{"p1":{"x":378,"y":491},"p2":{"x":428,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp983106908695176","type":"square","data":{"p1":{"x":428,"y":491},"p2":{"x":478,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp22919029527678036","type":"square","data":{"p1":{"x":428,"y":441},"p2":{"x":478,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp29968363685590615","type":"square","data":{"p1":{"x":478,"y":441},"p2":{"x":528,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3064750695507099","type":"square","data":{"p1":{"x":478,"y":491},"p2":{"x":528,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp20736005522617829","type":"square","data":{"p1":{"x":525,"y":491},"p2":{"x":575,"y":541}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6630182056016451","type":"square","data":{"p1":{"x":525,"y":441},"p2":{"x":575,"y":491}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6367769495837221","type":"square","data":{"p1":{"x":378,"y":541},"p2":{"x":428,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp45409685814242895","type":"square","data":{"p1":{"x":378,"y":591},"p2":{"x":428,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5545094435953948","type":"square","data":{"p1":{"x":428,"y":591},"p2":{"x":478,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5517734831857946","type":"square","data":{"p1":{"x":428,"y":541},"p2":{"x":478,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp20289578441162526","type":"square","data":{"p1":{"x":478,"y":541},"p2":{"x":528,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4020803982259509","type":"square","data":{"p1":{"x":478,"y":591},"p2":{"x":528,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp1766489111590892","type":"square","data":{"p1":{"x":525,"y":591},"p2":{"x":575,"y":641}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp16611246825798087","type":"square","data":{"p1":{"x":525,"y":541},"p2":{"x":575,"y":591}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4397254545171949","type":"square","data":{"p1":{"x":575,"y":241},"p2":{"x":625,"y":291}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp6144807074910452","type":"square","data":{"p1":{"x":575,"y":291},"p2":{"x":625,"y":341}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp3589652433184991","type":"square","data":{"p1":{"x":625,"y":291},"p2":{"x":675,"y":341}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp25892967213242923","type":"square","data":{"p1":{"x":625,"y":241},"p2":{"x":675,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp4183642206297993","type":"square","data":{"p1":{"x":675,"y":241},"p2":{"x":725,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp6199453733360385","type":"square","data":{"p1":{"x":675,"y":291},"p2":{"x":725,"y":341}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp8371298480252081","type":"square","data":{"p1":{"x":725,"y":291},"p2":{"x":775,"y":341}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp13406543930001424","type":"square","data":{"p1":{"x":725,"y":241},"p2":{"x":775,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp7028434611598733","type":"square","data":{"p1":{"x":575,"y":341},"p2":{"x":625,"y":391}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp9298084376936537","type":"square","data":{"p1":{"x":575,"y":391},"p2":{"x":625,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp17638628967307812","type":"square","data":{"p1":{"x":625,"y":391},"p2":{"x":675,"y":441}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp8659306906875608","type":"square","data":{"p1":{"x":625,"y":341},"p2":{"x":675,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp6760179239899888","type":"square","data":{"p1":{"x":675,"y":341},"p2":{"x":725,"y":391}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp4703731577764707","type":"square","data":{"p1":{"x":675,"y":391},"p2":{"x":725,"y":441}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp3902017727992544","type":"square","data":{"p1":{"x":725,"y":391},"p2":{"x":775,"y":441}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp8125113004618014","type":"square","data":{"p1":{"x":725,"y":341},"p2":{"x":775,"y":391}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp32227943902444856","type":"square","data":{"p1":{"x":775,"y":241},"p2":{"x":825,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp7046139495824904","type":"square","data":{"p1":{"x":775,"y":291},"p2":{"x":825,"y":341}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp2582360082210593","type":"square","data":{"p1":{"x":825,"y":291},"p2":{"x":875,"y":341}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp7234703671701124","type":"square","data":{"p1":{"x":825,"y":241},"p2":{"x":875,"y":291}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp224168987154868","type":"square","data":{"p1":{"x":875,"y":241},"p2":{"x":925,"y":291}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp4429037502051958","type":"square","data":{"p1":{"x":875,"y":291},"p2":{"x":925,"y":341}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp5934086888601495","type":"square","data":{"p1":{"x":775,"y":341},"p2":{"x":825,"y":391}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp34647497452059106","type":"square","data":{"p1":{"x":775,"y":391},"p2":{"x":825,"y":441}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp8838652582483997","type":"square","data":{"p1":{"x":825,"y":391},"p2":{"x":875,"y":441}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp39327584130580706","type":"square","data":{"p1":{"x":825,"y":341},"p2":{"x":875,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp25457308057723793","type":"square","data":{"p1":{"x":875,"y":341},"p2":{"x":925,"y":391}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp05157365310508544","type":"square","data":{"p1":{"x":875,"y":391},"p2":{"x":925,"y":441}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp6598923080433117","type":"square","data":{"p1":{"x":575,"y":441},"p2":{"x":625,"y":491}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8931837386821815","type":"square","data":{"p1":{"x":575,"y":491},"p2":{"x":625,"y":541}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8441801761893293","type":"square","data":{"p1":{"x":625,"y":491},"p2":{"x":675,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp1735650379366538","type":"square","data":{"p1":{"x":625,"y":441},"p2":{"x":675,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp9342397578745862","type":"square","data":{"p1":{"x":675,"y":441},"p2":{"x":725,"y":491}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp7694262302209971","type":"square","data":{"p1":{"x":675,"y":491},"p2":{"x":725,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp33906859025307123","type":"square","data":{"p1":{"x":725,"y":491},"p2":{"x":775,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp33387336474854434","type":"square","data":{"p1":{"x":725,"y":441},"p2":{"x":775,"y":491}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp08833313973544366","type":"square","data":{"p1":{"x":575,"y":541},"p2":{"x":625,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp43142666554992126","type":"square","data":{"p1":{"x":575,"y":591},"p2":{"x":625,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp05949538566313306","type":"square","data":{"p1":{"x":625,"y":591},"p2":{"x":675,"y":641}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp24816565159759318","type":"square","data":{"p1":{"x":625,"y":541},"p2":{"x":675,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8832394865589608","type":"square","data":{"p1":{"x":675,"y":541},"p2":{"x":725,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp8588819532959482","type":"square","data":{"p1":{"x":675,"y":591},"p2":{"x":725,"y":641}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp02822771621453768","type":"square","data":{"p1":{"x":725,"y":591},"p2":{"x":775,"y":641}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp24505768825868124","type":"square","data":{"p1":{"x":725,"y":541},"p2":{"x":775,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp9943831893798387","type":"square","data":{"p1":{"x":775,"y":441},"p2":{"x":825,"y":491}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp6622865692334068","type":"square","data":{"p1":{"x":775,"y":491},"p2":{"x":825,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp40445818778016873","type":"square","data":{"p1":{"x":825,"y":491},"p2":{"x":875,"y":541}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp30939585026857697","type":"square","data":{"p1":{"x":825,"y":441},"p2":{"x":875,"y":491}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp2809099477447172","type":"square","data":{"p1":{"x":875,"y":441},"p2":{"x":925,"y":491}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp42636709193771627","type":"square","data":{"p1":{"x":875,"y":491},"p2":{"x":925,"y":541}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp6263193537482754","type":"square","data":{"p1":{"x":775,"y":541},"p2":{"x":825,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp297853410797716","type":"square","data":{"p1":{"x":775,"y":591},"p2":{"x":825,"y":641}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp9146349458962533","type":"square","data":{"p1":{"x":825,"y":591},"p2":{"x":875,"y":641}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"dp058933813800658985","type":"square","data":{"p1":{"x":825,"y":541},"p2":{"x":875,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp6671617403492529","type":"square","data":{"p1":{"x":875,"y":541},"p2":{"x":925,"y":591}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp7954409637004844","type":"square","data":{"p1":{"x":875,"y":591},"p2":{"x":925,"y":641}},"style":{"fillColor":[208,2,27,0.15]}},{"id":"dp48513391766262703","type":"square","data":{"p1":{"x":-72,"y":341},"p2":{"x":-22,"y":391}},"style":{"fillColor":[208,2,27,0.4]}},{"id":"da3442923557518702","data":[{"x":900,"y":416},{"x":900,"y":516},{"x":850,"y":566},{"x":303,"y":566},{"x":153,"y":416},{"x":-147,"y":416}],"head":"*","tail":"*","shaft":"-","mVer":1,"style":{"thickness":6,"strokeColor":[144,19,254,1]}},{"id":"da5303496885296317","data":[{"x":-147,"y":416},{"x":153,"y":416},{"x":550,"y":566},{"x":850,"y":566},{"x":900,"y":516},{"x":900,"y":422}],"head":"no","tail":"no","shaft":{"type":"dash","pattern":[10,10]},"mVer":1,"style":{"thickness":6,"strokeColor":[126,211,33,1]}},{"id":"da008054528199299638","data":[{"x":253,"y":200},{"x":351.746337890625,"y":200}],"head":"no","tail":"no","shaft":"|","mVer":1,"style":{"thickness":5,"strokeColor":[139,87,42,1]},"settings":{"separatorDistance":34,"separatorLength":19}},{"id":"da17926097111239736","data":[{"x":646.753662109375,"y":200},{"x":720,"y":200}],"head":"no","tail":"no","shaft":{"type":"dash","pattern":[10,10]},"mVer":1,"style":{"thickness":6,"strokeColor":[126,211,33,1]}},{"id":"da4222432829281828","data":[{"x":458,"y":200},{"x":531.246337890625,"y":200}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":6,"strokeColor":[144,19,254,1]}},{"id":"dp17521394459649975","type":"square","data":{"p1":{"x":-220,"y":170},"p2":{"x":-170,"y":220}},"style":{"fillColor":[208,2,27,1]}},{"id":"dp5910416443524849","type":"square","data":{"p1":{"x":-10,"y":170},"p2":{"x":40,"y":220}},"style":{"fillColor":[208,2,27,0.4]}}],"settings":{"grid":true,"diagramHeight":797.2120971679688,"textSnapToGrid":true}}]},{"id":"n0.9915862430825819","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":71,"delayRenderCache":{"av":71,"map":{}}}

==> tikz_diagrams/docs/17747c85-5c3f-4404-939f-1a8dca6e0f86 <==
{"id":"321241621323","lines":[{"id":"n0.3851416450923924","blocks":[],"style":{"align":"center"}},{"id":"n0.1493432827626584","blocks":[{"id":"n0.14416636304379926","text":"\\diagram","type":"composite","elements":{"de7894807081399393":{"id":"de7894807081399393","lines":[{"id":"n0.24170902224599677","blocks":[{"id":"n0.2409438581015928","text":"Path","style":{"fontSize":"\\footnotesize"}}]}],"shape":{"data":{"p":{"x":105.43336636472881,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,1]}},"isTextMode":true,"isInGroup":true},"de7517301783189698":{"id":"de7517301783189698","lines":[{"blocks":[{"id":"n0.11888704593994337","text":"TASC","style":{"fontSize":"\\footnotesize"}}],"id":"n0.15878962547562647"}],"shape":{"data":{"p":{"x":148.26845089996306,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[245,166,35,1]}},"isTextMode":true,"isInGroup":true},"de19225636680799574":{"id":"de19225636680799574","lines":[{"blocks":[{"id":"n0.33854912358992406","text":"Ref","style":{"fontSize":"\\footnotesize"}}],"id":"n0.8895008907257687"}],"shape":{"data":{"p":{"x":187.1668318236441,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de5081123840764077":{"id":"de5081123840764077","lines":[{"blocks":[{"id":"n0.6995168912042349","text":"MIQP/MPC","style":{"fontSize":"\\footnotesize"}}],"id":"n0.9544965069554485"}],"shape":{"data":{"p":{"x":237.031744236652,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":true},"de21161580913428657":{"id":"de21161580913428657","lines":[{"blocks":[{"text":"MIQP/MPC","style":{"fontSize":"\\footnotesize"},"id":"n0.3336601991280388"}],"id":"n0.8681807145422649"}],"shape":{"data":{"p":{"x":551.031744236652,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":true},"de4071740344622663":{"id":"de4071740344622663","lines":[{"blocks":[{"text":"Ref","style":{"fontSize":"\\footnotesize"},"id":"n0.5180229021765814"}],"id":"n0.03508774291480177"}],"shape":{"data":{"p":{"x":501.1668318236441,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de10731628789245207":{"id":"de10731628789245207","lines":[{"blocks":[{"text":"TASC","style":{"fontSize":"\\footnotesize"},"id":"n0.0924202929276825"}],"id":"n0.7917350334982101"}],"shape":{"data":{"p":{"x":462.268450899963,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[245,166,35,1]}},"isTextMode":true,"isInGroup":true},"de012130312795047171":{"id":"de012130312795047171","lines":[{"blocks":[{"text":"Path","style":{"fontSize":"\\footnotesize"},"id":"n0.14501130212901958"}],"id":"n0.011554590086421346"}],"shape":{"data":{"p":{"x":419.43336636472884,"y":28.383093074774663},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,1]}},"isTextMode":true,"isInGroup":true},"de6288878311321933":{"id":"de6288878311321933","lines":[{"blocks":[{"text":"MIQP/MPC","style":{"fontSize":"\\footnotesize"},"id":"n0.010970578293059807"}],"id":"n0.22142173390262077"}],"shape":{"data":{"p":{"x":507.031744236652,"y":285.67842648987187},"rotation":0},"anchor":"center","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":true},"de4241679200693371":{"id":"de4241679200693371","lines":[{"blocks":[{"text":"Ref","style":{"fontSize":"\\footnotesize"},"id":"n0.3729866021858359"}],"id":"n0.7500174827037129"}],"shape":{"data":{"p":{"x":457.1668318236441,"y":285.67842648987187},"rotation":0},"anchor":"center","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de3114176410344456":{"id":"de3114176410344456","lines":[{"blocks":[{"text":"TASC","style":{"fontSize":"\\footnotesize"},"id":"n0.5523183430083958"}],"id":"n0.22940533974895816"}],"shape":{"data":{"p":{"x":418.26845089996306,"y":285.67842648987187},"rotation":0},"anchor":"center","style":{"fillColor":[245,166,35,1]}},"isTextMode":true,"isInGroup":true},"de9571941896100069":{"id":"de9571941896100069","lines":[{"blocks":[{"text":"Path","style":{"fontSize":"\\footnotesize"},"id":"n0.1232376882438222"}],"id":"n0.3927247830420244"}],"shape":{"data":{"p":{"x":359.43336636472884,"y":231.990339244582},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,1]}},"isTextMode":true,"isInGroup":true},"de07404466358905348":{"id":"de07404466358905348","lines":[{"blocks":[{"text":"MIQP/MPC","style":{"fontSize":"\\footnotesize"},"id":"n0.464994912990337"}],"id":"n0.10341787802807767"}],"shape":{"data":{"p":{"x":193.031744236652,"y":285.67842648987187},"rotation":0},"anchor":"center","style":{"fillColor":[80,227,194,1]}},"isTextMode":true,"isInGroup":true},"de2916453691851497":{"id":"de2916453691851497","lines":[{"blocks":[{"text":"Ref","style":{"fontSize":"\\footnotesize"},"id":"n0.6192125025935646"}],"id":"n0.6814577777575719"}],"shape":{"data":{"p":{"x":143.1668318236441,"y":285.67842648987187},"rotation":0},"anchor":"center","style":{"fillColor":[248,231,28,1]}},"isTextMode":true,"isInGroup":true},"de2903408186251575":{"id":"de2903408186251575","lines":[{"blocks":[{"text":"TASC","style":{"fontSize":"\\footnotesize"},"id":"n0.9616781206571006"}],"id":"n0.0025488552122072683"}],"shape":{"data":{"p":{"x":104.26845089996309,"y":285.67842648987187},"rotation":0},"anchor":"center","style":{"fillColor":[245,166,35,1]}},"isTextMode":true,"isInGroup":true},"de5046891350770186":{"id":"de5046891350770186","lines":[{"blocks":[{"text":"Path","style":{"fontSize":"\\footnotesize"},"id":"n0.09769915769942128"}],"id":"n0.12209904514778946"}],"shape":{"data":{"p":{"x":102.43336636472881,"y":231.990339244582},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,1]}},"isTextMode":true,"isInGroup":true},"de45472416280516637":{"id":"de45472416280516637","lines":[{"blocks":[{"text":"Path","style":{"fontSize":"\\footnotesize"},"id":"n0.8774909419171721"}],"id":"n0.16874562489898604"}],"shape":{"data":{"p":{"x":616.4333663647288,"y":231.990339244582},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,1]}},"isTextMode":true,"isInGroup":true},"de5781690567374516":{"id":"de5781690567374516","lines":[{"id":"n0.8948792142496136","blocks":[{"id":"n0.3976367876435549","text":"CPU"}]}],"shape":{"data":{"p":{"x":44.699991861979214,"y":259.42671391651004},"rotation":270},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de09427825002118939":{"id":"de09427825002118939","lines":[{"blocks":[{"id":"n0.7738227488629548","text":"thread 0"}],"id":"n0.5259287783674664"}],"shape":{"data":{"p":{"x":67.79999999999997,"y":29.752106982750767},"rotation":269.98},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de3789755470730025":{"id":"de3789755470730025","lines":[{"blocks":[{"text":"iteration ","style":{"fontSize":"\\footnotesize"},"id":"n0.2533767469905579"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathnormal"},"text":"k","id":"n0.9881523631938016"}],"id":"n0.08593046506970614"}],"id":"n0.38209397012651736"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\footnotesize"},"id":"n0.39778760301281135"}],"id":"n0.7525644179554098"}],"shape":{"data":{"p":{"x":85,"y":291.8141718334828},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de0352298465411367":{"id":"de0352298465411367","lines":[{"blocks":[{"text":"iteration ","style":{"fontSize":"\\footnotesize"},"id":"n0.8443828548446484"},{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"style":{"mathType":"\\mathnormal"},"text":"k","id":"n0.37288498600598685"},{"text":"+1","id":"n0.2775202807219048"}],"id":"n0.4417640461643708"}],"id":"n0.4230988446157422"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\footnotesize"},"id":"n0.901569881804559"},{"text":" ","style":{"fontSize":"\\footnotesize"},"id":"n0.4000311310162403"}],"id":"n0.9240055587994824"}],"shape":{"data":{"p":{"x":399.25,"y":291.8141718334828},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6263679006838863":{"id":"de6263679006838863","lines":[{"blocks":[{"text":"time","id":"n0.28954598353489747","style":{"fontSize":"\\footnotesize"}}],"id":"n0.4263808483721587"}],"shape":{"data":{"p":{"x":647.75,"y":292.3265123192656},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4510943713390254":{"id":"de4510943713390254","lines":[{"blocks":[{"text":"max. com. latency","id":"n0.9728865466165655"}],"id":"n0.10448855841210825"}],"shape":{"data":{"p":{"x":260,"y":267.9824686966207},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de36171824472460434":{"id":"de36171824472460434","lines":[{"blocks":[{"text":"time","id":"n0.7834783618623993","style":{"fontSize":"\\footnotesize"}}],"id":"n0.44556459672156157"}],"shape":{"data":{"p":{"x":647.75,"y":238.63842507397572},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4708167721475993":{"id":"de4708167721475993","lines":[{"blocks":[{"id":"n0.6060365631607294","text":"path planning period"}],"id":"n0.6360629699549718"}],"shape":{"data":{"p":{"x":173,"y":214.29438145133082},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de4095553517225825":{"id":"de4095553517225825","lines":[{"blocks":[{"text":"path planning period","id":"n0.788859709375539"}],"id":"n0.742937086116696"}],"shape":{"data":{"p":{"x":433.00000000000006,"y":214.29438145133082},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de771893004779739":{"id":"de771893004779739","lines":[{"blocks":[{"text":"thread 1","id":"n0.3359658336851019"}],"id":"n0.7541494817396643"}],"shape":{"data":{"p":{"x":65.79999999999997,"y":232.75210698275077},"rotation":269.98},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de007926188070065399":{"id":"de007926188070065399","lines":[{"blocks":[{"text":"thread 0","id":"n0.12048333996352611"}],"id":"n0.8069297448664232"}],"shape":{"data":{"p":{"x":65.8,"y":286.1478838619758},"rotation":269.98},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de2885444048686767":{"id":"de2885444048686767","lines":[{"id":"n0.44945880771230584","blocks":[{"id":"n0.5552888571475754","text":"iteration ","style":{"fontSize":"\\footnotesize"}},{"id":"n0.4700695569438007","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.5534718532445206","lines":[{"id":"n0.7706617343578877","blocks":[{"style":{"mathType":"\\mathnormal"},"id":"n0.8761607642350673","text":"k"}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\footnotesize"}}]}],"shape":{"data":{"p":{"x":88,"y":34.61548528337148},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8576355138114087":{"id":"de8576355138114087","lines":[{"blocks":[{"text":"iteration ","id":"n0.8118809124146238","style":{"fontSize":"\\footnotesize"}},{"id":"n0.3916959194287355","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.20582863287475983","lines":[{"blocks":[{"style":{"mathType":"\\mathnormal"},"text":"k","id":"n0.02399813008137186"},{"id":"n0.225951278764567","text":"+1"}],"id":"n0.9046137955167126"}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle","fontSize":"\\footnotesize"}},{"text":" ","id":"n0.1344524716058746","style":{"fontSize":"\\footnotesize"}}],"id":"n0.4871421199350532"}],"shape":{"data":{"p":{"x":402.25,"y":34.61548528337148},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9466501921559165":{"id":"de9466501921559165","lines":[{"blocks":[{"id":"n0.16429564157937393","text":"time","style":{"fontSize":"\\footnotesize"}}],"id":"n0.025946408810481048"}],"shape":{"data":{"p":{"x":650.75,"y":35.136611847789375},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de5365535768254195":{"id":"de5365535768254195","lines":[{"id":"n0.25496417789547476","blocks":[{"id":"n0.11981209977873042","text":"max. com. latency"}]}],"shape":{"data":{"p":{"x":285,"y":10.636615329371779},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true},"de3387333367631873":{"id":"de3387333367631873","lines":[{"blocks":[{"id":"n0.38504616563492644","text":"CPU"}],"id":"n0.9568631383934334"}],"shape":{"data":{"p":{"x":46.8,"y":29.75210698275076},"rotation":269.98},"anchor":"center","settings":{"fontSize":"\\footnotesize"}},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di5344856926018944","items":[],"style":{}},"shapes":[{"id":"dg04828865052291165","entities":[{"id":"da27260616801889515","data":[{"x":82.5,"y":36.3690075379686},{"x":680.3999938964844,"y":36.3690075379686}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dg21774650772835802","entities":[{"id":"dp6254808677683981","type":"rectangle","data":{"p1":{"x":85,"y":20.397178611580724},"p2":{"x":125.86673272945765,"y":36.3690075379686}},"style":{"fillColor":[126,211,33,1]}},{"id":"dl44846655092699983","linkedId":"de7894807081399393"}],"data":{"rotation":0}},{"id":"dg9837955877547309","entities":[{"id":"dp20611502122877678","type":"rectangle","data":{"p1":{"x":125.67927065271698,"y":20.397178611580724},"p2":{"x":170.85763114720913,"y":36.3690075379686}},"style":{"fillColor":[245,166,35,1]}},{"id":"dl8948327567503656","linkedId":"de7517301783189698"}],"data":{"rotation":0}},{"id":"dg23009359394783324","entities":[{"id":"dp6013625451332878","type":"rectangle","data":{"p1":{"x":170.67016907046852,"y":20.397178611580724},"p2":{"x":203.66349457681963,"y":36.3690075379686}},"style":{"fillColor":[248,231,28,1]}},{"id":"dl919024043838879","linkedId":"de19225636680799574"}],"data":{"rotation":0}},{"id":"dg5292822449737633","entities":[{"id":"dp09004847799634952","type":"rectangle","data":{"p1":{"x":203.66349457681963,"y":20.397178611580724},"p2":{"x":270.3999938964844,"y":36.3690075379686}},"style":{"fillColor":[80,227,194,1]}},{"id":"dl16818580548640472","linkedId":"de5081123840764077"}],"data":{"rotation":0}},{"id":"da2965898469364161","data":[{"x":85,"y":7.163370537980241},{"x":85,"y":48.233787777263345}],"head":"no","tail":"no","shaft":"--","mVer":1},{"id":"da6181327489608861","data":[{"x":398.9,"y":6.402807255771294},{"x":398.9,"y":47.473224495054396}],"head":"no","tail":"no","shaft":"--","mVer":1},{"id":"dg037779553086211726","entities":[{"id":"dp46636919295756774","type":"rectangle","data":{"p1":{"x":399,"y":20.397178611580724},"p2":{"x":439.86673272945757,"y":36.3690075379686}},"style":{"fillColor":[126,211,33,1]}},{"id":"dl9226463222314345","linkedId":"de012130312795047171"}],"data":{"rotation":0}},{"id":"dg04338784355267866","entities":[{"id":"dp254956499458036","type":"rectangle","data":{"p1":{"x":439.6792706527169,"y":20.397178611580724},"p2":{"x":484.8576311472091,"y":36.3690075379686}},"style":{"fillColor":[245,166,35,1]}},{"id":"dl4499234848579181","linkedId":"de10731628789245207"}],"data":{"rotation":0}},{"id":"dg10047317809950518","entities":[{"id":"dp13011297919250797","type":"rectangle","data":{"p1":{"x":484.67016907046855,"y":20.397178611580724},"p2":{"x":517.6634945768196,"y":36.3690075379686}},"style":{"fillColor":[248,231,28,1]}},{"id":"dl8019772140928025","linkedId":"de4071740344622663"}],"data":{"rotation":0}},{"id":"dg9350893487023884","entities":[{"id":"dp4520264049297906","type":"rectangle","data":{"p1":{"x":517.6634945768196,"y":20.397178611580724},"p2":{"x":584.3999938964844,"y":36.3690075379686}},"style":{"fillColor":[80,227,194,1]}},{"id":"dl9612751502228625","linkedId":"de21161580913428657"}],"data":{"rotation":0}},{"id":"da7692662711274847","data":[{"x":271.3999938964844,"y":27.698579157621797},{"x":399.3999938964844,"y":27.698579157621797}],"head":">","tail":"<","shaft":"--","mVer":1},{"id":"dp527200541215572","type":"rectangle","data":{"p1":{"x":57.399993896484375,"y":2.9042231207749563},"p2":{"x":695.3999938964844,"y":56.59998388156176}}},{"id":"dp11514131696089192","type":"rectangle","data":{"p1":{"x":19.95211613802419,"y":19.25210698275078},"p2":{"x":73.6478838619758,"y":40.25210698275077},"rotation":270}},{"id":"dg7013369985031974","entities":[{"id":"dp7941276062688329","type":"rectangle","data":{"p1":{"x":40.952116138024174,"y":19.252106982750778},"p2":{"x":94.64788386197577,"y":40.25210698275076},"rotation":270}},{"id":"dl2348225039683498","linkedId":"de09427825002118939"}]},{"id":"dl5292022640733924","linkedId":"de2885444048686767"},{"id":"dl5557380167488657","linkedId":"de8576355138114087"},{"id":"dl8204181023101782","linkedId":"de9466501921559165"},{"id":"dl24851195693992056","linkedId":"de5365535768254195"},{"id":"dl73686746565317","linkedId":"de3387333367631873"}]},{"id":"dg4370302653825555","entities":[{"id":"da7340458845450337","data":[{"x":79.5,"y":293.61821404023163},{"x":677.3999938964844,"y":293.61821404023163}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dg7810281723496169","entities":[{"id":"dp7231047008758391","type":"rectangle","data":{"p1":{"x":82,"y":224.0505516942222},"p2":{"x":122.86673272945765,"y":239.93012679494174}},"style":{"fillColor":[126,211,33,1]}},{"id":"dl24939744219683058","linkedId":"de5046891350770186"}],"data":{"rotation":0}},{"id":"dg8762657178046211","entities":[{"id":"dp10198375010095218","type":"rectangle","data":{"p1":{"x":81.679270652717,"y":277.7386389395121},"p2":{"x":126.8576311472091,"y":293.61821404023163}},"style":{"fillColor":[245,166,35,1]}},{"id":"dl76721623913319","linkedId":"de2903408186251575"}],"data":{"rotation":0}},{"id":"dg4907261552355935","entities":[{"id":"dp5902638169258501","type":"rectangle","data":{"p1":{"x":126.67016907046852,"y":277.7386389395121},"p2":{"x":159.6634945768196,"y":293.61821404023163}},"style":{"fillColor":[248,231,28,1]}},{"id":"dl05966413671002946","linkedId":"de2916453691851497"}],"data":{"rotation":0}},{"id":"dg2858679093699603","entities":[{"id":"dp7982729754436804","type":"rectangle","data":{"p1":{"x":159.6634945768196,"y":277.7386389395121},"p2":{"x":226.39999389648435,"y":293.61821404023163}},"style":{"fillColor":[80,227,194,1]}},{"id":"dl03556419500669761","linkedId":"de07404466358905348"}],"data":{"rotation":0}},{"id":"da7635124884455893","data":[{"x":81.7,"y":264.5812697902563},{"x":81.7,"y":305.41446290639226}],"head":"no","tail":"no","shaft":"--","mVer":1},{"id":"da686617272726473","data":[{"x":395.6,"y":263.82509954736486},{"x":395.6,"y":304.65829266350084}],"head":"no","tail":"no","shaft":"--","mVer":1},{"id":"dg9010457443536293","entities":[{"id":"dp28586314481223773","type":"rectangle","data":{"p1":{"x":339,"y":224.0505516942222},"p2":{"x":379.8667327294577,"y":239.93012679494174}},"style":{"fillColor":[126,211,33,1]}},{"id":"dl9809518505145409","linkedId":"de9571941896100069"}],"data":{"rotation":0}},{"id":"dg6393887897758503","entities":[{"id":"dp46931067795436854","type":"rectangle","data":{"p1":{"x":395.679270652717,"y":277.7386389395121},"p2":{"x":440.8576311472092,"y":293.61821404023163}},"style":{"fillColor":[245,166,35,1]}},{"id":"dl10351713706555143","linkedId":"de3114176410344456"}],"data":{"rotation":0}},{"id":"dg7773374933669956","entities":[{"id":"dp13207370055736334","type":"rectangle","data":{"p1":{"x":440.67016907046855,"y":277.7386389395121},"p2":{"x":473.66349457681963,"y":293.61821404023163}},"style":{"fillColor":[248,231,28,1]}},{"id":"dl19586320635254517","linkedId":"de4241679200693371"}],"data":{"rotation":0}},{"id":"dg9066549005435101","entities":[{"id":"dp7442275256466211","type":"rectangle","data":{"p1":{"x":473.66349457681963,"y":277.7386389395121},"p2":{"x":540.3999938964844,"y":293.61821404023163}},"style":{"fillColor":[80,227,194,1]}},{"id":"dl9035669773653474","linkedId":"de6288878311321933"}],"data":{"rotation":0}},{"id":"da7158696174850716","data":[{"x":226.39999389648435,"y":284.9978663483243},{"x":396.3999938964844,"y":284.9978663483243}],"head":">","tail":"<","shaft":"--","mVer":1},{"id":"da7308496107605746","data":[{"x":79.5,"y":239.93012679494174},{"x":677.3999938964844,"y":239.93012679494174}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dg1965323975677684","entities":[{"id":"dp16188381476159042","type":"rectangle","data":{"p1":{"x":596,"y":224.0505516942222},"p2":{"x":636.8667327294577,"y":239.93012679494174}},"style":{"fillColor":[126,211,33,1]}},{"id":"dl052622752270977236","linkedId":"de45472416280516637"}],"data":{"rotation":0}},{"id":"da14847441731609679","data":[{"x":123.39999389648438,"y":231.3097791030344},{"x":339.3999938964844,"y":231.3097791030344}],"head":">","tail":"<","shaft":"--","mVer":1},{"id":"da6576169033456851","data":[{"x":379.39999389648443,"y":231.3097791030344},{"x":595.3999938964844,"y":231.3097791030344}],"head":">","tail":"<","shaft":"--","mVer":1},{"id":"dp7298789693686925","type":"rectangle","data":{"p1":{"x":55.389346687643354,"y":205.90246586482846},"p2":{"x":693.3893466876434,"y":259.2880780900164}}},{"id":"dp7895786578903246","type":"rectangle","data":{"p1":{"x":55.389346687643354,"y":259.5905531101183},"p2":{"x":693.3893466876434,"y":312.9761653353063}}},{"id":"dg22966590998806025","entities":[{"id":"dp4318482185112418","type":"rectangle","data":{"p1":{"x":-8.799052822587868,"y":248.92671391651004},"p2":{"x":98.19903654654624,"y":269.92671391651004},"rotation":270}},{"id":"dl4429631884723726","linkedId":"de5781690567374516"}],"data":{"rotation":0}},{"id":"dp09397064563515678","type":"rectangle","data":{"p1":{"x":38.952116138024174,"y":222.25210698275077},"p2":{"x":92.64788386197577,"y":243.25210698275077},"rotation":270}},{"id":"dp21628070883737416","type":"rectangle","data":{"p1":{"x":38.952116138024195,"y":275.6478838619758},"p2":{"x":92.6478838619758,"y":296.6478838619758},"rotation":270}},{"id":"dl6579003855331385","linkedId":"de3789755470730025"},{"id":"dl22836203133716793","linkedId":"de0352298465411367"},{"id":"dl5136653265910585","linkedId":"de6263679006838863"},{"id":"dl12353940618486736","linkedId":"de4510943713390254"},{"id":"dl5270028236376674","linkedId":"de36171824472460434"},{"id":"dl5102040897274931","linkedId":"de4708167721475993"},{"id":"dl5415331790372662","linkedId":"de4095553517225825"},{"id":"dl5839391486958487","linkedId":"de771893004779739"},{"id":"dl42986016806342087","linkedId":"de007926188070065399"}]}],"settings":{"grid":true,"diagramHeight":404.20001220703125,"gridBold":false}}]},{"id":"n0.93463936609768","blocks":[],"style":{"align":"center"}}],"pageSettings":{"pageSize":{"width":700}},"delayRenderCache":{"av":792,"map":{}},"___version":2,"version":2,"av":792}

==> tikz_diagrams/docs/a375fd4c-dd65-4f69-8e7d-26cf335e88f8 <==
{"id":"r0.14202330469511082","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de366200392032515":{"id":"de366200392032515","lines":[{"id":"n0.4922084900437773","blocks":[{"id":"n0.16958838002815124","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.07755941093378516","lines":[{"id":"n0.12653506958358518","blocks":[{"id":"n0.19347627227518527","text":"r"},{"id":"n0.2751776904267511","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.35741858660575154","lines":[{"id":"n0.4718896624400415","blocks":[{"id":"n0.4042409539438858","text":"\\text","type":"composite","elements":{"textValue":{"id":"n0.23395658153098586","lines":[{"id":"n0.7678464166992471","blocks":[{"id":"n0.8921605336284908","text":"agent"}]}]}}}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":179,"y":310}},"anchor":"left-top"},"isTextMode":true},"de11232858258878053":{"id":"de11232858258878053","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"r","id":"n0.58103759461073"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"\\text","type":"composite","elements":{"textValue":{"lines":[{"blocks":[{"text":"agent","id":"n0.2778900039088936"}],"id":"n0.4927525669775381"}],"id":"n0.5471086153003679"}},"id":"n0.7286131720399747"}],"id":"n0.7965406167261719"}],"id":"n0.7581834436642121"}},"id":"n0.3781992450661793"}],"id":"n0.756909037787374"}],"id":"n0.8483821713500836"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.9228216357684942"}],"id":"n0.5105031391755457"}],"shape":{"data":{"p":{"x":401,"y":335}},"anchor":"left-top"},"isTextMode":true},"de20064028115095378":{"id":"de20064028115095378","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.2065918351461833","text":"z"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"\\text","type":"composite","elements":{"textValue":{"lines":[{"blocks":[{"id":"n0.4874677496451991","text":"offset"}],"id":"n0.21071862123565976"}],"id":"n0.6440546581470272"}},"id":"n0.5027631603374891"}],"id":"n0.47377638384324805"}],"id":"n0.5440238056346984"}},"id":"n0.5974537632690069"}],"id":"n0.8939169666790987"}],"id":"n0.9396879135935727"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7010511938146939"}],"id":"n0.16704838406618672"}],"shape":{"data":{"p":{"x":332,"y":185}},"anchor":"left-top"},"isTextMode":true},"de551392510838691":{"id":"de551392510838691","lines":[{"blocks":[{"id":"n0.706013749154712","text":"Sphere model"}],"id":"n0.7008651481814956"}],"shape":{"data":{"p":{"x":225,"y":125},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,0.1]}},"isTextMode":true,"isInGroup":true},"de8075617046874344":{"id":"de8075617046874344","lines":[{"blocks":[{"text":"Ellipsoid model","id":"n0.8676688123482545"}],"id":"n0.1032091807179274"}],"shape":{"data":{"p":{"x":435,"y":125},"rotation":0},"anchor":"center","style":{"fillColor":[126,211,33,0.1]}},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di6469837643957062","items":[],"style":{}},"shapes":[{"id":"dp7742717274641506","type":"image","data":{"p1":{"x":197,"y":204},"p2":{"x":257,"y":264},"url":"data-resources/f1f62b34-9bbd-4bbc-b772-5599a048e7f3"}},{"id":"dp6488663695379986","type":"circle","data":{"p1":{"x":168,"y":174},"p2":{"x":284.8702469152521,"y":290.8702469152521}},"style":{"fillColor":[126,211,33,0.1]}},{"id":"dp5060359038216102","type":"ellipse","data":{"p1":{"x":168.80318061024573,"y":214.01327549274598},"p2":{"x":283.9968754105393,"y":253.63395541964633},"rotation":356.2,"skewX":27.04},"style":{"strokeType":"--"}},{"id":"da26773835711954264","data":[{"x":170,"y":310},{"x":230,"y":310}],"head":"|","tail":"|","shaft":"-","mVer":1},{"id":"dp685043000236766","type":"image","data":{"p1":{"x":419.2015417718981,"y":204},"p2":{"x":479.2015417718981,"y":264},"url":"data-resources/e982839e-c227-4e9f-993e-2d7288f6e81a"}},{"id":"dp9776969299541947","type":"ellipse","data":{"p1":{"x":391.0047223821439,"y":214.01327549274598},"p2":{"x":506.1984171824375,"y":253.63395541964633},"rotation":356.2,"skewX":27.04},"style":{"strokeType":"--"}},{"id":"da908679491853353","data":[{"x":392,"y":335},{"x":452,"y":335}],"head":"|","tail":"|","shaft":"-","mVer":1},{"id":"dp05121709873126812","type":"ellipse","data":{"p1":{"x":390.1664463246646,"y":149},"p2":{"x":507.0366932399167,"y":319}},"style":{"fillColor":[126,211,33,0.1]}},{"id":"da05612326774385257","data":[{"x":377,"y":149},{"x":377,"y":239}],"head":"|","tail":"|","shaft":"-","mVer":1},{"id":"dp5694086777545051","type":"rectangle","data":{"p1":{"x":150,"y":110},"p2":{"x":300,"y":370}}},{"id":"dp1646208152406834","type":"rectangle","data":{"p1":{"x":320,"y":110},"p2":{"x":550,"y":370}}},{"id":"dg5483258116250034","entities":[{"id":"dp4051444957890875","type":"rectangle","data":{"p1":{"x":150,"y":110},"p2":{"x":300,"y":140}},"style":{"fillColor":[126,211,33,0.1]}},{"id":"dl29411001588822105","linkedId":"de551392510838691"}],"data":{}},{"id":"dg5282297525223882","entities":[{"id":"dp34024466509469664","type":"rectangle","data":{"p1":{"x":320,"y":110},"p2":{"x":550,"y":140}},"style":{"fillColor":[126,211,33,0.1]}},{"id":"dl011817195988081286","linkedId":"de8075617046874344"}],"data":{}}],"settings":{"grid":true,"diagramHeight":924.2750244140625,"textSnapToGrid":true},"id":"n0.6513005200058133"}],"id":"n0.3987484649743718"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":535,"delayRenderCache":{"av":535,"map":{}}}

==> tikz_diagrams/general_pipeline_modifications.tex <==
\draw (356.95,750.9) node  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{100.34pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Generate Time-Aware Safe Corridors around the global path}
\end{center}

\draw (135,716) node  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{80.76pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Create potential field and find a path to the goal}
\end{center}
